Coffee: Boost Your Code LLMs by Fixing Bugs with Feedback

Code editing is an essential step towards reliable program synthesis to automatically correct critical errors generated from code LLMs. Recent studies have demonstrated that closed-source LLMs (i.e., ChatGPT and GPT-4) are capable of generating corrective feedback to edit erroneous inputs. However, it remains challenging for open-source code LLMs to generate feedback for code editing, since these models tend to adhere to the superficial formats of feedback and provide feedback with misleading information. Hence, the focus of our work is to leverage open-source code LLMs to generate helpful feedback with correct guidance for code editing. To this end, we present Coffee, a collected dataset specifically designed for code fixing with feedback. Using this dataset, we construct CoffeePots, a framework for COde Fixing with FEEdback via Preference-Optimized Tuning and Selection. The proposed framework aims to automatically generate helpful feedback for code editing while minimizing the potential risk of superficial feedback. The combination of Coffee and CoffeePots marks a significant advancement, achieving state-of-the-art performance on HumanEvalFix benchmark. Codes and model checkpoints are publicly available at https://github.com/Lune-Blue/COFFEE.

==> 1_intro_dump.tex <==
\section{Introduction}

% promising ability of code llms, but code editing still remains a challenge

% necessity of bug fix
%Thus, training LLMs to automatically correct errors in source codes is an important next step in code-related tasks~\citep{}. 



\begin{comment}
    [1문단]
    code LLM이 생성한 code는 suboptimal => code editing 중요
    [2문단]
    최근 연구들은 LLM이 feedback을 통해서 editing 능력을 향상시킬 수 있는 promising한 ability가 있다는 점을 보여줌
    하지만 이런 ability는 closed-source LLM (e.g., ChatGPT and GPT-4)에만 한정되어있으며 security vulnarabilities, lack of transparency 같은 문제가 있음
    따라서 open-source model에도 이러한 ability를 endow할 수 있는 방법에 대한 연구가 필요함.
    [3문단]
    quality feedback을 잘 생성하도록 배우는 것은 nontrivial (figure 1)
    [4문단]
    our strategy (유지)
\end{comment}

Thanks to extensive pretraining on code corpora, large language models (LLMs)~\citep{brown2020gpt3} have shown significant success on code generation~\citep{tyers-etal-2023-codex}. 
However, these large language models (LLMs) of code, \ie, code LLMs, usually generate source codes containing bugs that lead to undesirable outputs~\citep{ekbal2022adversarial}.
Hence the task of \textbf{code editing}, which aims to automatically correct errors in codes without human effort~\citep{wei2023coeditor,gupta2020repair}, is an important step in building a reliable programming assistant such as 
Copilot\footnote{\url{https://github.com/features/copilot}}.
% Copilot~\citep{copilot}.

\input{figure_latex/motivating_example}

% code llms need feedback to deal with critical errors in the given source code.

%In this paper, we propose an alternative approach called Reflexion that uses verbal reinforcement to help agents learn from prior failings. Reflexion converts binary or scalar feedback from the environment into verbal feedback in the form of a textual summary, which is then added as additional context for the LLM agent in the next episode. This self-reflective feedback acts as a ‘semantic’ gradient signal by providing the agent with a concrete direction to improve upon, helping it learn from prior mistakes to perform better on the task. This is akin to how humans iteratively learn to accomplish complex tasks in a few-shot manner – by reflecting on their previous failures in order to form an improved plan of attack for the next attempt. For example, in figure 1, a Reflexion agent learns to optimize its own behavior to solve decision-making, programming, and reasoning tasks through trial, error, and self-reflection.

%The task requires the model to first localize critical error spans in the source code and then suggest correct solutions to the problem, as illustrated in Figure~\ref{fig:motivate}. 
Prior studies~\citep{shinn2023reflexion, madaan2023selfrefine} have shown that LLMs demonstrate promising capabilities of generating feedback to correct errors in an erroneous input. However, most of these approaches depend solely on closed-source LLMs (\eg, ChatGPT and GPT-4~\citep{openai2023chatgpt, openai2023gpt4}) to generate corrective feedback for code editing, limiting their use for research and industrial purposes due to high costs and potential security risks~\citep{bommasani2022opportunities}. Motivated by this, we explore alternative approaches that leverage open-source code LLMs to provide feedback for better code editing performance.
%Prior works suggest that such large language models are not yet capable of correcting code when lacking external feedback, such as unit tests or human instructions (Chen et al., 2023a).
 % ~\footnote{\url{https://openai.com/blog/chatgpt}}


Generating corrective feedback for erroneous source codes poses a challenge to open-source code LLMs. 
The problem lies in that the code LLMs are pre-trained on tasks that are misaligned with the goal of code editing. 
While recent work seeks to close this gap by training code LLMs to follow instructions~\citep{roziere2023code}, 
these instructions do not usually include detailed explanations for error correction, rendering them less suitable for code editing.
As a result, the code LLMs tend to generate plausible feedback with unhelpful information, leading to suboptimal edits from code editing models as illustrated in Figure~\ref{fig:motivate}.


%This motivates us to devise a strategy to curate helpful feedback that contains correct solutions to key errors while avoiding misleading feedback from the code LLMs.

%While more recent approaches aim at enhancing understanding of source codes by training code LLMs to follow instruction~\citep{},
%Such feedback either lacks explanations on critical errors in the source code or suggests incorrect solutions to the problem
%since the task requires the models to locate errors in an incorrect code and make edits to repair such erro

To address this issue, we present \coffee \textbf{\textsc{Coffee}}, a dataset curated for \textbf{CO}de \textbf{F}ixing with \textbf{FEE}dback. 
Our dataset is constructed from edit histories in competitive programming platforms such that the collected dataset reflects the general pattern of error correction from human users. Using a closed-source LLM, we annotate corrective feedback for incorrect solutions and apply several filters to ensure the quality of the annotated dataset. 

%Our dataset differs from the conventional code corpora in that it contains task-specific feedback curated to tackle errors in buggy source codes. 
Using the collected dataset, we construct \textbf{\textsc{CoffeePots}}, a framework for \textbf{CO}de \textbf{F}ixing with \textbf{FEE}dback via \textbf{P}reference-\textbf{O}ptimized \textbf{T}uning and \textbf{S}election. 
Our framework consists of a critic model to generate feedback, an editor to edit codes based on the feedback, and a feedback selector to choose the best possible feedback from the critic. 
The intuition behind our design is that we (1) \textit{sample} multiple plausible feedback candidates from the critic and (2) \textit{select} the most helpful feedback for the editor. 
To improve the helpfulness of the feedback, we further align it with the model preference of the editor via preference tuning on the critic and preference selection from feedback selector. 
Our experiments show that \textbf{\textsc{CoffeePots}} produces helpful feedback for the code editing model and achieves state-of-the-art performance on code editing benchmarks.

Our contributions are threefold: (1) We present \coffee \textbf{\textsc{Coffee}}, a high-quality dataset targeted for code editing with feedback. (2) We propose \textbf{\textsc{CoffeePots}}, a framework for code editing with feedback that achieves state-of-the-art performance by providing helpful feedback for code editing. (3) We conduct extensive analysis on \textbf{\textsc{CoffeePots}} to validate the effectiveness of our approach. 

\begin{comment}
%%%%% We need feedback for code editing %%%%%
% Why feedback? What makes code editing challenging without feedback?
% Code editing models require guidance to find optimal solution for the given problem.
%%% code llm fails to generate the right solution when given question + wrong solution
%%%%% Hypothesis 1) The discrepancy between generation and editing?
%%%%% Hypothesis 2) LLMs do not understand which kind of error is in the source code.
%%%%% >> no knowledge of how different errors appear in an actual source code?
%%%%% >> no knowledge of which errors lead to more critical failure in the given code.
% a handful of errors that require 


% Problems that lead to two conclusions
%%% code editing models require feedback to identify and correct errors in the given source code. [improving the quality of the feedback ]
%%% iterative feedback is required to maximally  

\end{comment}

\begin{comment}
%%%%% Providing code LLMs with feedback %%%%%
% Challenge: how do we make sure we provide best feedback possible to our code editing model, given that it is hard to obtain optimal feedback
% what is a good feedback = correctly addresses the critical failures in the given source code.
\end{comment}



\begin{comment}
%%%%% Iterative code editing framework with feedback %%%%%
% Our framework includes a critic model that is trained to produce high-quality feedback for the subsequent editing model
% We also include a feedback selector that selects the best possible feedback to minimize the negative effect from suboptimal feedback. 
% With iterative feedback, , closing the gap between open-source and close-sourced models.  (close-???) 
\end{comment}


\begin{comment}
    왜 피드백이 필요한가, 즉 왜 틀린 코드에서 바로 correct code 로 가는 것보다 피드백을 생성하는 것이 유용한가. 틀린 코드를 수정하려면 2 step 이 필요하다. 먼저 틀린 부분을 짚고, 그 부분을 수정하는 과정이 필요하다. 틀린 부분을 찾는 것의 난이도가 높은데, 여기서 동시에 그 부분을 수정하는 과정까지 학습하는 것은 굉장히 어려운 난이도이다.
\end{comment}

\begin{comment}
    % achieves competitive .. results under much smaller budget constraint.    
\end{comment}

==> 4_experiment_dump.tex <==



\section{Experimental Settings}
\subsection{Datasets}
\label{ssec:datasets}
\input{tables/main_humanevalfix}

We evaluate the effectiveness of \textsc{CoffeePots} for code editing under two scenarios.
First, we test \textsc{CoffePots} on a benchmark for code editing task with a particular focus on assessing the code editing capability.
For that, we use HumanEvalFix~\citep{muennighoff2023octopack}, which is designed to check whether the models is capable of fixing various types of error in the codes.
%First, focusing more on assessing code editing ability itself, we test \textsc{CoffePots} on a benchmark for code editing task.
%For that, we use HumanEvalFix~\citep{muennighoff2023octopack}, which is designed to have various types of error in the codes, and the goal is to fix them.
Secondly, we further explore whether \textsc{CoffeePots} can boost the code generation performance of code LLMs by editing errors in the output code. 
We prompt the code generation models to provide a solution for each problem $q$ from the following three benchmarks for code generation:
HumanEvalSynthesize~\citep{muennighoff2023octopack}, APPS~\citep{hendrycksapps2021}, and MBPP~\cite{austin2021program}.
%We prompt code LLMs to generate a solution for each problem $q$ from the following three benchmarks for code generation: HumanEvalSynthesize~\citep{muennighoff2023octopack}, APPS~\citep{hendrycksapps2021}, and MBPP~\cite{austin2021program}.  


% We assess the effectiveness of \textsc{CoffeePots} for code editing under two practical scenarios. 
% First, we evaluate model performance in editing codes written by humans.
% For that, we adopt HumanEvalFix~\citep{muennighoff2023octopack}, a benchmark for code editing that contains human-written codes with various errors for programming problems from HumanEval~\citep{chen2021codex}.

% Secondly, we adopt \textsc{CoffeePots} to edit wrong codes generated by machines. To elicit machine-generated codes, we prompt ChatGPT~\citep{openai2023chatgpt} to generate a solution (\ie, code) for each problem $q$ from the following three benchmark datasets for code generation:
% HumanEvalSynthesize~\citep{muennighoff2023octopack}, APPS~\citep{hendrycksapps2021}, and MBPP~\cite{austin2021program}.  

\input{tables/main_codegen}
\subsection{Metrics}
Following prior studies~\citep{muennighoff2023octopack,chen2021codex}, we report the code editing performance using pass@1, which is the percentage of problems in the test set that the model solves in a single attempt.
For code generation benchmarks, we additionally report Error-Resolved Rate (ERR), which measures how many errors are addressed via editing.
Specifically, we compute ERR as the proportion of correct edits among problems with incorrect solutions from the generation model.\footnote{ERR is equivalent to pass@1 in code editing benchmarks since all problems are annotated with incorrect solutions. See Appendix~\ref{appendix:benchmarks} for more details on benchmarks and metrics.}


%\input{tables/chatgpt_error_detection}
%\paragraph{Discrepancy between two scenarios.}

%\paragraph{Understanding the different results under two experimental settings.}
% To demonstrate the difference since detecting and resolving errors from the codes generated by ChatGPT is more challenging compared to the codes annotated in HumanEvalFix. We conduct an analysis to measure the difficulty of identifying error 
% While \textsc{CoffeePots} significantly outperforms the closed-source baselines in the code editing benchmark, in the code generation benchmarks, it shows comparable or slightly lower performance compared to the closed-source baselines.


\begin{comment}
%is solved by the predicted solution. 
Along with this metric, we introduce Error-Resolved Rate (ERR), which aims to measure how many errors have been resolved via editing.
% the impact of editing on pass@1.
Specifically, we compute ERR by dividing the gain in pass@1 from editing by 100 minus the pass@1 score before editing, and then multiplying the result by 100.~\footnote{We only apply ERR on the code generation benchmarks. Because in the code editing benchmark, pass@1 before editing will be 0, resulting same score to pass@1. }
% how much editing is effective in improving the solution for the code. 
% expressing this difference as a ratio of the potential improvement relative to the initial pass@1 score.
% ERR is calculates as $(\text{pass@1 after editing} - \text{pass@1 before editing})/(100 - \text{pass@1 before editing})*100$.
% (Pass@1 of  Edit model - Pass@1 of Generation model)/ (100 - Pass@1 of Generation model)*100 = (75-67)/(100-67)*100

% For code generation benchmarks, we additionally report Error-Resolved Rate (ERR), which measures how many errors have been resolved via editing.
% Specifically, we compute ERR as the proportion of problems where the code genration model produces incorrect solutions and the code editing model correctly edits them.
\end{comment}

\subsection{Baselines}
We choose both \textbf{open-source} and \textbf{closed-source} LLMs as our baselines. For open-source baselines, we use popular foundation models for code-related tasks, including variants of StarCoder~\citep{li2023starcoder}, such as WizardCoder~\citep{luo2023wizardcoder} and OctoCoder, and CodeLlama family~\citep{roziere2023code}.
We also consider two closed-source baselines, ChatGPT~\citep{openai2023chatgpt} and GPT-4~\citep{openai2023gpt4}, which are only accessible via API. Our hypothesis is that \textsc{CoffeePots} significantly enhances the code editing capabilities of open-source models and shows performance competitive to the closed-source baselines.

We further consider two prompting methods to implement baselines that incorporate feedback into code-related tasks: (1) Self-Debug~\citep{chen2023teaching} is a method specialized in fixing bugs by incorporating \textbf{compiler feedback} (\eg{}, unit test results).
(2) Self-Refine~\citep{madaan2023selfrefine} uses \textbf{natural language feedback} to iteratively refine models' outputs.
These prompting techniques have shown that they can effectively push LLMs' performance forward in various tasks by using feedback.

\begin{comment}
We categorize baselines under two different criteria: accessibility and usage of feedback.

\paragraph{Accessibility.}
We use both open-source methods and closed-source methods as our baselines.
As we propose \textsc{CoffeePots} to mitigate the limitations of open-source model,
% Considering that \textsc{CoffeePots} is an open-source model,
we focus more on comparing it with open-source baselines than closed-source baselines.
For open-source baselines, we use popular foundation models for code-related tasks, including variants of StarCoder~\citep{li2023starcoder}, such as WizardCoder~\citep{luo2023wizardcoder} and OctoCoder, and CodeLlama family~\citep{roziere2023code}.
We also consider two closed-source baselines, ChatGPT~\citep{openai2023chatgpt} and GPT-4~\citep{openai2023gpt4}, which are only accessible via API. 
% While these models demonstrate strong performance in code-related tasks thanks to their large number of parameters~\citep{openai2023gpt4, liu2023your}, they do not permit further parameter updates.
% We include more details on the baselines, in Appendix~\ref{appendix:experimental_details}. 

\paragraph{Usage of feedback.}
In addition to the baselines without using feedback, we adopt two prompting methods as baselines that also use feedback, similar to ours: (1) Self-Debug~\citep{chen2023teaching} is a method specialized in fixing bugs by incorporating \textbf{compiler feedback} (\eg{}, unit test results).
(2) Self-Refine~\citep{madaan2023selfrefine} uses \textbf{natural language feedback} to iteratively refine models' outputs.
These prompting techniques have shown that they can effectively push LLMs' performance forward in various tasks by using feedback.
% refine~\citep{madaan2023selfrefine}, prompting methods that utilizes natural language and compiler feedback, respectively.
% To baselines that uses feedback
% Among open-source models, OctoCoder~\citep{muennighoff2023octopack} achieves the SOTA performance on HumanEvalFix~\citep{köpf2023oasst}.

% We also consider two closed-source baselines, ChatGPT and GPT-4, which are only accessible via API. 
% While these models demonstrate strong performance in code-related tasks thanks to their large number of parameters~\citep{openai2023gpt4, liu2023your}, they are trained on general-domain corpora and do not permit further parameter updates.
% We include more details on datasets and baselines, including the analysis of train-test overlap, in Appendix~\ref{appendix:experimental_details}. 
% We first consider \textbf{open-source} baselines, which are code LLMs whose parameters are made publicly available. 
% Among open-source models, OctoCoder~\citep{muennighoff2023octopack} achieves the SOTA performance on HumanEvalFix~\citep{köpf2023oasst}.
% We also consider two closed-source baselines, ChatGPT and GPT-4, which are only accessible via API. 
% While these models demonstrate strong performance in code-related tasks thanks to their large number of parameters~\citep{openai2023gpt4, liu2023your}, they are trained on general-domain corpora and do not permit further parameter updates.
% We include more details on datasets and baselines, including the analysis of train-test overlap, in Appendix~\ref{appendix:experimental_details}.
\end{comment}

\begin{comment}
    We employ both \textbf{open-} and \textbf{closed-source} baselines.
Open-source baselines are pre-trained LLMs additionally fine-tuned with code corpora. 
Among open-source baselines, OctoCoder~\citep{muennighoff2023octopack} is the SOTA model on HumanEvalFix.

For the closed-source baselines, we adopt ChatGPT and GPT-4. 
While these closed-source LLMs have exhibited strong performance in code-related tasks thanks to the large number of parameters~\citep{openai2023gpt4, liu2023your}, they 
are trained on general-domain corpora and do not permit further parameter updates.
\end{comment}

==> 5_results_dump.tex <==
\section{Experimental Results}
\subsection{Performance in Code Editing}

\paragraph{Code editing benchmark.}
Table~\ref{tab:humanevalfix} reports model performances (pass@1) in code editing on HumanEvalFix.
We observe that \textsc{CoffeePots} shows significantly higher performance than all open-source baselines, including those with larger parameter sizes.
Moreover, \textsc{CoffeePots} even outperforms the closed-source LLMs (\ie, ChatGPT and GPT-4), achieving SOTA performance on the HumanEvalFix benchmark. 
These results demonstrate \textsc{CoffeePots}'s efficacy in generating helpful feedback for successful code editing.

\input{tables/line_level_accuracy}
\input{tables/error_type}

\paragraph{Code generation benchmark.}
In this setting, the models are tasked to edit the codes generated by code generation models for code generation benchmarks (\cref{ssec:datasets}).
% In this setting, the models are tasked to edit the wrong codes generated by ChatGPT for benchmarks of code generation (\cref{ssec:datasets}).
% Here, we use \textbf{OctoCoder} and \textbf{ChatGPT} as baselines for code editing.
% Also, when using ChatGPT to edit wrong codes, we further augment it with: (1) \textbf{compiler feedback} sampled from the Python compiler following \citet{zhang2023selfedit}; (2) \textbf{natural language feedback} generated by ChatGPT based on given wrong codes.
The results are shown in Table~\ref{tab:codegen}.
\textsc{CoffeePots} outperforms all open-source baselines, including Code Llama (13B), the previous SOTA among open-source code LLMs.
Furthermore, \textsc{CoffeePots} shows better results than feedback-augmented Code Llama (13B), \ie{}, prompted with Self-Refine and Self-Debug, suggesting the effectiveness of our strategy on generating feedback.
% and even Code Llama (13B) prompted to utilize augmented natural language and compiler feedback.
In addition, while some open-source code LLMs show almost no improvement in MBPP and APPS (\ie{}, ERR is 0\%), \textsc{CoffeePots} shows meaningful improvements on these benchmarks.
% From the results, 
% Table~\ref{tab:codegen} shows that \textsc{CoffeePots} (7B) outperforms open-source baselines, and exhibits comparable performance to ChatGPT augmented with feedback. 
Compared to closed-source baselines (\ie{}, ChatGPT), \textsc{CoffeePots} shows comparable results on HumanEvalSythesize and MBPP and a slightly lower performance in APPS. 
% We posit that this is due to the difference in the capabilities obtained during pre-training, as APPS is specially designed to target more challenging problems.
% For APPS, which contains more challenging problems compared to others, closed-source baselines show slightly stronger performance compared to \textsc{CoffeePots}.
These demonstrate that our framework can serve as an alternative to closed-source LLMs while being publicly available and much smaller in size, which are crucial in real-world application.
%While using ChatGPT for code editing yields much improvement in pass@1, \textsc{CoffeePots} achieves performance competitive to ChatGPT with diverse feedback. 
%reveal the strong capability of \textsc{CoffeePots} in code editing that is even competitive to closed-source LLM with significantly more parameters.
%Also, \textsc{CoffeePots} achieves best performance on HumanEvalSynth and MBPP benchmarks and shows comparable performance in APPS benchmark when compared with closed-source LLMs with various approaches. 
% \paragraph{Understanding the mixed results from two types of benchmarks.}

\begin{comment}
\input{tables/chatgpt_error_detection}
\paragraph{Understanding the different results under two experimental settings.}
We observe that the increase in pass@1 over the baselines is slightly smaller in the code generation benchmark than in the code editing benchmark. 
First, this is due to the difference in the portion of target code for editing. While in code editing benchmarks, all solutions are considered for editing, we only edit solutions tested as erroneous by running example test cases in the code generation benchmarks (\eg{}, 51\% in MBPP).
To compensate the difference between two experimental settings, we introduce ERR, which shows the impact of editing more clearly.

Secondly, detecting and resolving errors from the codes generated by ChatGPT is more challenging compared to the codes annotated in HumanEvalFix. We conduct an analysis to measure the difficulty of identifying error 
% While \textsc{CoffeePots} significantly outperforms the closed-source baselines in the code editing benchmark, in the code generation benchmarks, it shows comparable or slightly lower performance compared to the closed-source baselines.
\end{comment}


\begin{comment}
To better understand the different results from code editing and code generation benchmarks, we conduct human evaluation that assesses the correctness of feedback from ChatGPT on erroneous codes.\footnote{Details on the human evaluation are in Appendix~\ref{appendix:human_error_detection}.} The evaluation results and ERR on the two settings are shown in Table~\ref{tab:error_detection_and_err}. 
Compared to the code editing benchmark (\ie{}, HumanEvalFix), the feedback on the three code generation benchmarks shows relatively lower correctness. The results suggest that it is more challenging to identify errors in the code generation benchmarks, resulting lower ERR for both ChatGPT and \textsc{CoffeePots}.
\end{comment}

\begin{comment}
\paragraph{Discrepancy between code editing and generation.}
\paragraph{Challenges in editing machine-generated codes.}
\paragraph{Understanding the different results under two experimental settings.}
We observe that the increase in pass@1 over the baselines is slightly smaller in the code generation benchmark than in the code editing benchmark. 

Secondly, detecting and resolving errors from the codes generated by ChatGPT is more challenging compared to the codes annotated in HumanEvalFix. In Table~\ref{} we present an analysis to measure the difficulty of identifying error 
% While \textsc{CoffeePots} significantly outperforms the closed-source baselines in the code editing benchmark, in the code generation benchmarks, it shows comparable or slightly lower performance compared to the closed-source baselines.
\end{comment}


% We find that \textsc{CoffeePots} significantly outperforms both open-source and closed-source baselines in the code editing benchmark, but obtain somewhat mixed results from the code generation benchmarks.
% To better understand the results, we conduct in-depth analysis to explain the reason.

% We provide an analysis that helps to understand the results of two categories of benchmarks.
% While \textsc{CoffeePots} significantly outperforms open-source baselines and even closed-source baselines in a large margin on the code editing benchmark, the results on code generation benchmarks seem a bit different.
% \textsc{CoffeePots} has shown that it can 
% Since we adopt two different evaluation settings (\ie{}, code editing benchmark and code generation benchmark), to assess code editing ability of \textsc{CoffeePots}, they have shown somewhat different 

\subsection{Analyses on the Effect of Feedback}
\paragraph{Error detection.}
To examine whether feedback
from \textsc{CoffeePots} helps the editor better detect errors,
we measure the error detection rates of editing models on HumanEvalFix to approximate how well these models locate critical errors in a source code. 
The error detection rate is computed as the number of edited error lines divided by the number of total error lines in the wrong code. 
In Table~\ref{tab:line_accuracy}, we observe that \textsc{CoffeePots} shows a significantly higher detection rate than both open- and closed-source baselines, suggesting that augmenting the editor with feedback benefits the model in the localization of errors.

%Secondly, we further explore whether \textsc{CoffeePots} can boost the code generation performance of code LLMs by editing errors in the output code. 


\paragraph{Error types.} Table~\ref{table:error_type} breaks down the performance of open- and closed-source LLMs on HumanEvalFix by different error types. 
We observe that \textsc{CoffeePots} shows particularly strong performance on problems with excess logic or value/operator misuse, which require models to locate the exact error spans. 
We also find that our approach achieves performance comparable to GPT-4 on problems with missing logic, indicating that augmenting our editor with feedback improves understanding of the implicit logic in source codes. 
Overall, \textsc{CoffeePots} consistently surpasses open-source baselines for all error types. In Appendix~\ref{appendix:case_study}, we present empirical examples and case studies of feedback/editing from \cpemoji~\textsc{CoffeePots}.

%We note that while \textsc{CoffeePots} shows lower performance than GPT-4 on problems with function misuse, these problems can only be addressed with specific knowledge on programming, which is only attainable via LLMs with exceptionally large size. 

\begin{comment}
    Humanevalfix dataset은 6 error type을 contain 하고 있음
    우리의 모델이 어떤 error type을 잘 하는지 분석하기위해 각 error type별로 pass@1 score를 계산했다
    우리는 특히
    operator misuse (34.0%)
    excess logic(25.8 %)
    variable misuse (21.8 %)
    에서 더 높은 성능향상을 보이며, 
    missing logic (12.1%)
    value misuse (11.3%)
    function misuse (same)
    
    6가지 에러 타입이 있는데(각 에러 타입을 간단하게 설명), [굳이 해야하나?]
    octocoder 의 결과와 비교했을때 우리가 logic 에 대한 문제들을 더 잘 수정하는 것을 알 수 있다. 
    Missing logic: Misses code needed to solve the problem
    Excess logic: Contains excess code leading to mistakes
    Value misuse: incorrect value is used
    Operator misuse: incorrect operator is used
    Variable misuse: incorrect variable is used
    Function misuse: incorrect function is used
\end{comment}

%\subsection{Feedback Quality}


%\subsection{Importance of Feedback Quality}
\begin{comment}
    GPT4 feedback, ours(critic-editor), low quality feedback(negative sampling 을 통해 다른 문제에 대한 feedback 을 사용하는 셋팅)
    GPT4 feedback: 61.7
    ours: 38.4
    low quality feedback: 25.6 
\end{comment}
% human evaluation

%\subsection{Importance of Selector}
\begin{comment}
    Oracle feedback, ours(only feedback selector), random selected feedback 을 비교
    Oracle feedback selector: 66.4
    ours: 45.1
    random selected feedback: 39.6
\end{comment}

\subsection{Ablation Studies}\label{analysis:ablation_study}
\input{tables/ablation}
We conduct ablation studies to investigate the effectiveness of each component in \textsc{CoffeePots}. Here, we consider the following ablations: (1) \textbf{Supervised Fine-tuning (SFT)}: a vanilla critic model trained with only SFT (\cref{ssec:sft}). (2) \textbf{Preference tuning}: a vanilla (SFT) critic that further goes through preference-tuning (\cref{ssec:dpo}) without feedback selection. (3) \textbf{Feedback selection}: a vanilla critic model paired with a feedback selector (\cref{ssec:feedback_selector}) that selects the best feedback candidates from it. 

\paragraph{Preference alignment benefits code editing.}\label{analysis:helpful_feedback}
Table~\ref{table:ablation} compares the pass@1 performance on the HumanEvalFix benchmark of each setting.
We see a decrease in code editing performance when the editor is provided with feedback from the SFT critic model, 
which is in line with the finding that critic trained with only SFT fails to generate feedback for correct solutions. 
On the contrary, we observe that applying preference tuning and feedback selection on the SFT critic model leads to significant performance gain from the editor, demonstrating the effectiveness of our approach. 

\paragraph{Preference alignment improves the quality of feedback.}
We conjecture that aligning feedback with the preference of the editor largely improves its quality. To validate this, we follow \citet{liu2023geval} and prompt GPT-4 to conduct pair-wise comparison on feedback from \textsc{CoffeePots}
and its variants using the prompt in Table~\ref{tab:gpt4_compare_prompt}. 
Figure~\ref{fig:g-eval} shows that for 47$\%$ of the test cases, \textsc{CoffeePots} produces feedback with higher quality than the SFT critic. 
Notably, we find that applying preference tuning largely improves the likelihood of generating high-quality feedback, as the win percentage of \textsc{CoffeePots} decreases from 47.0$\%$ to 23.8$\%$. 

\input{figure_latex/g_eval}
\input{figure_latex/feedback_quality}
\paragraph{Feedback selector leaves out unhelpful feedback.}
We also observe in Figure~\ref{fig:g-eval} that applying feedback selection over the SFT critic moderately improves the feedback quality. 
To see how feedback quality benefits from feedback selection,
we measure the helpfulness of feedback from \textsc{CoffeePots} and the preference-tuned critic via GPT-4 and compare their distribution in Figure~\ref{fig:feedback_quality}. We see that applying the feedback selector to the preference-tuned critic (\ie, \textsc{CoffeePots}) largely reduces the number of low-quality feedback from the critic model, effectively improving the overall quality of the generated feedback.\footnote{See Appendix~\ref{appendix:experimental_details} for experimental details.}

\begin{comment}
우리는 피드백, DPO, Selector 의 효과를 알아보기 위해 ablation study 를 진행하였다. 그것에 대한 결과는 table ?? 에 있다. 우리의 observation 은 다음과 같다. 1. 단순히 피드백을 사용하는 것은 오히려 피드백을 사용하는 것만 못하다. -> 피드백의 퀄리티가 중요하다는걸 얘기할 수 있지 않을까  3. Selector 를 통해 생성된 피드백 중 optimal(?) 한 피드백을 고르는 것이 도움이 되는 것을 관측했다. 4. DPO 와 Selector 를 함께 사용하는 것이 큰 도움이 되는 것을 확인했으며, 이를 통해 GPT-4 의 성능을 넘었다. 
줄이고, 두 문단, DPO 와 selector 는 orthogonal 하다 -> 함께 적용하면 더 오름
\end{comment}


% Following \citet{liu2023geval}, we leverage GPT-4 to score feedback based on each following aspect and compare feedback.
% \begin{itemize}
%     \item Clarity: Does the feedback correctly identify the error in the code?
%     \item Accuracy: Does feedback provide a technically accurate explanation of the mistake?
%     \item Validity: Is it possible to correct from incorrect code to correct code by using feedback?
% \end{itemize}
% The comparison results are illustrated in Figure~\ref{fig:g-eval}. Compared to the other three settings, \textsc{CoffeePots} shows a higher feedback quality. However, the advantage of our framework's feedback becomes less marked compared to Preference tuning and Feedback selection, indicating an enhancement in feedback quality. Remarkably, the winning percentage of \textsc{CoffeePots} decreases significantly when compared to preference tuning, while making a substantially high proportion of ties. This suggests that preference tuning significantly improves the quality of feedback. 

\begin{comment}
    말하고자 하는 내용: 다른 세가지 세팅에 비해 우리의 프레임워크가 더 높은 피드백의 퀄리티를 보여줌. 하지만, preference tuning 을 진행했을때와 feedback selector 를 사용했을 때 우리 프레임워크의 피드백이 더 좋은 비율이 줄어들면서, preference tuning 과 feedback selector 의 적용을 통해 피드백 퀄리티가 상승했음을 보여줌. 특히, Preference tuning 을 진행한 결과와 비교했을 때 다른 비교 결과와 달리 우리 모델의 win ratio 가 감소하고 Tie 의 비율이 굉장히 높은 것을 확인할 수 있는데, 이를 통해 preference tuning 이 피드백 퀄리티를 크게 올렸음을 알 수 있다. 
\end{comment}


\begin{comment}
우리는 octocoder 와 우리 모델 간의 iterative 성능을 비교하였다. (왜 비교했을까..) 피규어 결과에서 알 수 있듯이, 우리 모델이 octocoder 를 매 iteration 마다 크게 이기는 것을 확인할 수 있다. 또한 우리가 제시한 프레임워크를 사용하지 않는 셋팅에서는(without coffeepot) 각 iteration 마다 성능이 크게 밀리는 것을 볼 수 있다.
\end{comment}

==> 6_conclusion_dump.tex <==

Large language models have shown a promising ability to correct their output by generating feedback. However, this ability is only limited to closed-source models, which raises concerns regarding cost and security.
% In this paper, we aim to build an open-source model that can generate feedback to correct errors in source codes.
To this end, we present \textsc{Coffee}, a dataset collected for code fixing with feedback.
% To train a model to produce helpful feedback that can guide the editing, we first collect a dataset for code fixing with annotated feedback, named \textsc{Coffee}.
However, we find that supervised finetuning on the dataset resorts to producing unhelpful feedback.
To resolve this issue, we introduce \textsc{CoffeePots},
% Since helpfulness of feedback is critical 
% This work addresses generating high-quality feedback in order to leverage the instruction-following capabilities of code LLMs. 
% To this end, we present \textsc{Coffee}, a dataset for code fixing with annotated feedback. 
a framework that aligns feedback with the model's preference which improves the helpfulness of feedback.
% a framework that significantly improves the model's code-fixing capabilities, achieving state-of-the-art performance on HumanEvalFix benchmark. 
Through extensive experiments, we demonstrate that \textsc{CoffeePots} outperforms all baselines, achieving state-of-the-art performance.
% and exhibits robustness against various error types.
% can be further applied to iterative editing by leveraging feedback.

%최근 연구들은 LLM이 feedback을 통해서 editing 능력을 향상시킬 수 있는 promising한 ability가 있다는 점을 보여줌, 하지만 quality feedback을 잘 생성하도록 배우는 것은 nontrivial
% This work address generating high-quality feedback in order to leverage the instruction-following capabilities of CodeLLM. We present COFFEE, a dataset for code fixing with feedback annotated by ChatGPT. We present COFFEEPOTs, a framework that significantly improves the model's code-fixing capabilities, achieving State-of-the-art performance on HumanEvalFix benchmark. Through extensive experiments, we demonstrate that our proposed framework exhibits robustness against various types of error types and can effectively fix codes through iterative editing by leveraging feedback.

In this paper, we aim to build an open-source model that can generate feedback to correct errors in source codes.
To train a model to produce helpful feedback that can guide the editing we first collect a dataset for code fixing with annotated feedback, named \textsc{Coffee}.
However, we find that supervised finetuning on the dataset resorts to producing superficial feedback.
To resolve this issueend, we introduce \textsc{CoffeePots},
% Since helpfulness of feedback is critical 
% This work addresses generating high-quality feedback in order to leverage the instruction-following capabilities of code LLMs. 
% To this end, we present \textsc{Coffee}, a dataset for code fixing with annotated feedback. 
a framework that aligns feedback with the edit model's preference which improves the helpfulness of feedback.
% a framework that significantly improves the model's code-fixing capabilities, achieving state-of-the-art performance on HumanEvalFix benchmark. 
Through extensive experiments, we demonstrate that \textsc{CoffeePots} outperforms all baselines, achieving state-of-the-art performance.
% and exhibits robustness against various error types.
% can be further applied to iterative editing by leveraging feedback.

This paper aims to enhance code editing with open-sourced code LLMs by automatically generating helpful feedback. To this end, we present \textsc{Coffee}, a task-specific for code fixing with feedback annotations. We also propose \textsc{CoffeePots},
a framework designed to further enhance the helpfulness of feedback by aligning feedback generation with the model preference of the code editor. 
Through extensive experiments, we demonstrate that \textsc{CoffeePots} achieves state-of-the-art performance on the code-editing benchmark by providing the code editor with helpful feedback.

% Since helpfulness of feedback is critical 
% This work addresses generating high-quality feedback in order to leverage the instruction-following capabilities of code LLMs. 
% To this end, we present \textsc{Coffee}, a dataset for code fixing with annotated feedback. 

==> tables/taxonomy.tex <==

\begin{table*}[t]
    %\centering
    %\small
    %\begin{tabular}{lccccc}
    %    \toprule
    %    \multicolumn{6}{c}{Related work on reasoning and decision-making} \\
    %    \toprule
    %    \textbf{ Approach} &
    %    \textbf{Self} &
    %    \textbf{ Hidden } &
    %    \textbf{Decision } &
    %    \textbf{Binary } & 
    %    \textbf{Memory} \\
    %    & \textbf{refine} & \textbf{constraints} & \textbf{making} & \textbf{reward} & \\
    %    \midrule
    %     Self-refine \citep{madaan2023self} & \greencheck & \redcross & \redcross & \redcross & %\redcross \\
    %     Beam search \citep{xie2023decomposition} & \greencheck & \greencheck & \greencheck & %\greencheck & \redcross \\
    %     \textbf{Reflexion (ours)} & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck %\\
    %\end{tabular}

    % Feedback
    % Task-specific
    % s

    % 
    % CommtiPack
    % \textsc{Coffee}
    
    \centering
    \small
    \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}{*}{\textbf{Approach}} & \textbf{Code-targeted}& {\textbf{Diverse}}  & \textbf{Submission}  & \textbf{Test} & \textbf{Diverse} & \textbf{Natural language} \\
        & \textbf{dataset} & \textbf{difficulty}  & \textbf{history}  & \textbf{cases} & \textbf{solutions} & \textbf{feedback} \\
        \midrule
        CommitPack \citep{chen2023teaching} & \greencheck & \redcross & \redcross & \redcross & \redcross & \redcross \\ % & \redcross \\
        MBPP \citep{austin2021program} & \greencheck & \redcross & \redcross & \greencheck & \redcross &\redcross \\ % & \\
        APPS \citep{hendrycksapps2021} & \greencheck & \greencheck & \redcross & \redcross & \greencheck & \redcross \\ %& \redcross \\
        %\hline
        FixEval \citep{haque2023fixeval} & \greencheck & \greencheck & \redcross & \greencheck &\greencheck & \redcross \\
        %\hline
        \textbf{\textsc{Coffee}} & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck \\
        %\greencheck \\
        \bottomrule
    \end{tabular}
    %\vspace{-10pt}
    \caption{A taxonomy of different datasets for code-related tasks. }
    \label{tab:taxonomy}
\end{table*}
